Playing the network backward: A Game Theoretic Attribution Framework

Attribution methods explain which input features drive a model's prediction, making them central to model debugging and mechanistic interpretability. Yet backward attribution methods, including gradients, LRP, and transformer-specific rules, lack a shared framework in which to compare the underlying backward calculations. We introduce such a framework by recasting backward attribution as a two-player game on an extended network graph, building on Gaubert and Vlassopoulos' ReLU Net Game. Gradients and the full alpha-beta-LRP family arise as integrals over game trajectories under specific equilibria, so attribution maps become projections of trajectory distributions rather than the primary object. Desired explanation properties, such as localisation focus, robustness to input noise, or stable attention routing, can be specified as game-theoretic concepts, including policy regularization, risk aversion, and extended action sets, and translate directly into novel adaptations of the well-known backward rules. On ViT-B/16, one such selected adaptation of alpha-beta-LRP outperforms prior transformer-specific backward methods across all considered localisation metrics.

==> tables/generated/ablations_resnet50_longtable.tex <==
\begin{longtable}{@{}l l c c c c c c c@{}}
\toprule
Center & Factor & Value & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ \\
\midrule
\endfirsthead
\toprule
Center & Factor & Value & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ \\
\midrule
\endhead
\bottomrule
\endlastfoot
RG (faith) & $\tau$ & 0.3 & 0.688 & 0.727 & 0.684 & 6.10 & 5.10 & 4.357 \\
 &  & 0.4 & 0.676 & 0.712 & 0.692 & 6.08 & 5.03 & 4.340 \\
 &  & 0.5 & 0.677 & 0.720 & 0.706 & 6.06 & 5.00 & 4.308 \\
 &  & 0.6 & 0.673 & 0.704 & 0.711 & 5.99 & 4.96 & 4.270 \\
 &  & 0.7 & 0.667 & 0.680 & 0.707 & 5.95 & 4.89 & 4.219 \\
 &  & 0.8 & 0.665 & 0.688 & 0.711 & 5.89 & 4.85 & 4.134 \\
 &  & 0.9 & 0.674 & 0.720 & 0.728 & 5.88 & 4.79 & 4.075 \\
 &  & \textbf{1} & 0.674 & 0.743 & 0.738 & 5.88 & 4.74 & 4.030 \\
\midrule
RG (faith) & $\lambda$ & {-}5 & 0.667 & 0.740 & 0.730 & 5.90 & 4.81 & 4.034 \\
 &  & {-}2 & 0.672 & 0.740 & 0.736 & 5.89 & 4.75 & 4.034 \\
 &  & \textbf{{-}1} & 0.674 & 0.743 & 0.738 & 5.88 & 4.74 & 4.030 \\
 &  & {-}0.3 & 0.674 & 0.747 & 0.739 & 5.87 & 4.75 & 4.026 \\
 &  & 0 & 0.675 & 0.747 & 0.740 & 5.86 & 4.74 & 4.023 \\
\midrule
RG (faith) & $\sigma^2$ & \textbf{1} & 0.674 & 0.743 & 0.738 & 5.88 & 4.74 & 4.030 \\
 &  & 2 & 0.673 & 0.742 & 0.737 & 5.87 & 4.74 & 4.032 \\
 &  & 5 & 0.671 & 0.736 & 0.736 & 5.88 & 4.75 & 4.031 \\
 &  & 10 & 0.670 & 0.747 & 0.734 & 5.89 & 4.76 & 4.031 \\
\midrule
RG (faith) & $\varepsilon$ & 0.1 & 0.658 & 0.745 & 0.722 & 5.90 & 4.79 & 4.049 \\
 &  & \textbf{0.25} & 0.674 & 0.743 & 0.738 & 5.88 & 4.74 & 4.030 \\
 &  & 0.5 & 0.692 & 0.747 & 0.754 & 5.86 & 4.72 & 4.023 \\
 &  & 1 & 0.712 & 0.766 & 0.761 & 5.85 & 4.72 & 4.038 \\
\midrule
RG (loc) & $\tau$ & 0.3 & 0.733 & 0.761 & 0.719 & 6.03 & 5.04 & 4.272 \\
 &  & 0.4 & 0.717 & 0.758 & 0.718 & 6.02 & 4.96 & 4.243 \\
 &  & 0.5 & 0.709 & 0.740 & 0.720 & 5.98 & 4.92 & 4.216 \\
 &  & 0.6 & 0.710 & 0.733 & 0.728 & 5.93 & 4.87 & 4.172 \\
 &  & 0.7 & 0.716 & 0.745 & 0.741 & 5.91 & 4.80 & 4.125 \\
 &  & 0.8 & 0.720 & 0.761 & 0.752 & 5.87 & 4.72 & 4.078 \\
 &  & \textbf{0.9} & 0.719 & 0.763 & 0.760 & 5.85 & 4.70 & 4.047 \\
 &  & 1 & 0.713 & 0.770 & 0.763 & 5.85 & 4.70 & 4.035 \\
\midrule
RG (loc) & $\lambda$ & {-}5 & 0.708 & 0.765 & 0.745 & 5.89 & 4.80 & 4.069 \\
 &  & {-}2 & 0.716 & 0.773 & 0.755 & 5.87 & 4.74 & 4.055 \\
 &  & {-}1 & 0.718 & 0.777 & 0.757 & 5.86 & 4.72 & 4.054 \\
 &  & {-}0.3 & 0.719 & 0.768 & 0.758 & 5.86 & 4.72 & 4.050 \\
 &  & \textbf{0} & 0.719 & 0.763 & 0.760 & 5.85 & 4.70 & 4.047 \\
\midrule
RG (loc) & $\varepsilon$ & 0.1 & 0.656 & 0.712 & 0.712 & 5.89 & 4.84 & 4.106 \\
 &  & 0.25 & 0.674 & 0.717 & 0.730 & 5.87 & 4.77 & 4.067 \\
 &  & 0.5 & 0.696 & 0.736 & 0.749 & 5.84 & 4.70 & 4.042 \\
 &  & \textbf{1} & 0.719 & 0.763 & 0.760 & 5.85 & 4.70 & 4.047 \\
\end{longtable}


==> tables/generated/ablations_vgg16_longtable.tex <==
\begin{longtable}{@{}l l c c c c c c c@{}}
\toprule
Center & Factor & Value & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ \\
\midrule
\endfirsthead
\toprule
Center & Factor & Value & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ \\
\midrule
\endhead
\bottomrule
\endlastfoot
RG (faith) & $\tau$ & 0.3 & 0.685 & 0.736 & 0.673 & 14.48 & 9.64 & 5.632 \\
 &  & 0.4 & 0.645 & 0.657 & 0.641 & 14.40 & 9.36 & 5.574 \\
 &  & 0.5 & 0.626 & 0.653 & 0.628 & 14.27 & 9.14 & 5.451 \\
 &  & 0.6 & 0.633 & 0.651 & 0.646 & 14.07 & 9.00 & 5.258 \\
 &  & 0.7 & 0.643 & 0.671 & 0.674 & 14.03 & 8.98 & 5.142 \\
 &  & \textbf{0.8} & 0.640 & 0.712 & 0.688 & 14.05 & 9.07 & 5.117 \\
 &  & 0.9 & 0.630 & 0.742 & 0.693 & 14.05 & 9.17 & 5.126 \\
 &  & 1 & 0.618 & 0.749 & 0.695 & 14.06 & 9.25 & 5.137 \\
\midrule
RG (faith) & $\lambda$ & {-}5 & 0.518 & 0.458 & 0.536 & 17.60 & 13.82 & 7.362 \\
 &  & {-}2 & 0.623 & 0.604 & 0.631 & 15.90 & 11.58 & 5.852 \\
 &  & {-}1 & 0.636 & 0.676 & 0.661 & 15.03 & 10.35 & 5.404 \\
 &  & {-}0.3 & 0.640 & 0.694 & 0.676 & 14.54 & 9.70 & 5.231 \\
 &  & \textbf{0} & 0.640 & 0.712 & 0.688 & 14.05 & 9.07 & 5.117 \\
\midrule
RG (faith) & $\varepsilon$ & \textbf{0.1} & 0.640 & 0.712 & 0.688 & 14.05 & 9.07 & 5.117 \\
 &  & 0.25 & 0.639 & 0.692 & 0.684 & 14.18 & 9.23 & 5.146 \\
 &  & 0.5 & 0.638 & 0.690 & 0.680 & 14.34 & 9.46 & 5.183 \\
 &  & 1 & 0.639 & 0.690 & 0.676 & 14.63 & 9.79 & 5.249 \\
\midrule
RG (loc) & $\tau$ & \textbf{0.3} & 0.685 & 0.736 & 0.673 & 14.48 & 9.64 & 5.632 \\
 &  & 0.4 & 0.645 & 0.657 & 0.641 & 14.40 & 9.36 & 5.574 \\
 &  & 0.5 & 0.626 & 0.653 & 0.628 & 14.27 & 9.14 & 5.451 \\
 &  & 0.6 & 0.633 & 0.651 & 0.646 & 14.07 & 9.00 & 5.258 \\
 &  & 0.7 & 0.643 & 0.671 & 0.674 & 14.03 & 8.98 & 5.142 \\
 &  & 0.8 & 0.640 & 0.712 & 0.688 & 14.05 & 9.07 & 5.117 \\
 &  & 0.9 & 0.630 & 0.742 & 0.693 & 14.05 & 9.17 & 5.126 \\
 &  & 1 & 0.618 & 0.749 & 0.695 & 14.06 & 9.25 & 5.137 \\
\midrule
RG (loc) & $\lambda$ & {-}5 & 0.561 & 0.543 & 0.555 & 17.05 & 13.21 & 6.898 \\
 &  & {-}2 & 0.657 & 0.696 & 0.634 & 15.31 & 10.80 & 5.885 \\
 &  & {-}1 & 0.674 & 0.735 & 0.656 & 14.85 & 10.13 & 5.731 \\
 &  & {-}0.3 & 0.680 & 0.727 & 0.666 & 14.66 & 9.87 & 5.675 \\
 &  & \textbf{0} & 0.685 & 0.736 & 0.673 & 14.48 & 9.64 & 5.632 \\
\midrule
RG (loc) & $\varepsilon$ & \textbf{0.1} & 0.685 & 0.736 & 0.673 & 14.48 & 9.64 & 5.632 \\
 &  & 0.25 & 0.691 & 0.747 & 0.673 & 14.66 & 9.91 & 5.659 \\
 &  & 0.5 & 0.697 & 0.742 & 0.672 & 14.87 & 10.19 & 5.705 \\
 &  & 1 & 0.702 & 0.742 & 0.671 & 15.13 & 10.55 & 5.767 \\
\midrule
SG (faith) & $\lambda$ & {-}2 & 0.614 & 0.710 & 0.636 & 18.17 & 14.83 & 6.941 \\
 &  & {-}1 & 0.609 & 0.750 & 0.697 & 17.91 & 13.87 & 6.517 \\
 &  & \textbf{{-}0.3} & 0.598 & 0.821 & 0.788 & 17.08 & 12.98 & 6.278 \\
 &  & 0 & 0.547 & 0.781 & 0.764 & 17.63 & 14.35 & 6.789 \\
\midrule
SG (faith) & $\sigma^2$ & \textbf{1} & 0.598 & 0.821 & 0.788 & 17.08 & 12.98 & 6.278 \\
 &  & 2 & 0.601 & 0.811 & 0.765 & 17.30 & 13.07 & 6.323 \\
 &  & 5 & 0.604 & 0.798 & 0.731 & 17.66 & 13.50 & 6.417 \\
 &  & 10 & 0.607 & 0.763 & 0.706 & 17.86 & 13.77 & 6.500 \\
\midrule
SG (faith) & gate $\tilde\Phi$ & \textbf{off} & 0.598 & 0.821 & 0.788 & 17.08 & 12.98 & 6.278 \\
 &  & on & 0.568 & 0.823 & 0.805 & 17.30 & 13.74 & 6.428 \\
\midrule
SG (loc) & $\lambda$ & {-}5 & 0.568 & 0.550 & 0.558 & 18.17 & 14.31 & 7.509 \\
 &  & {-}2 & 0.620 & 0.703 & 0.681 & 17.84 & 13.63 & 6.404 \\
 &  & \textbf{{-}1} & 0.597 & 0.770 & 0.770 & 17.28 & 13.32 & 6.217 \\
 &  & {-}0.3 & 0.566 & 0.830 & 0.809 & 17.33 & 13.75 & 6.452 \\
 &  & 0 & 0.554 & 0.827 & 0.802 & 17.55 & 14.16 & 6.618 \\
\midrule
SG (loc) & $\sigma^2$ & 1 & 0.596 & 0.793 & 0.766 & 17.32 & 13.35 & 6.246 \\
 &  & 2 & 0.597 & 0.786 & 0.766 & 17.31 & 13.34 & 6.232 \\
 &  & \textbf{5} & 0.597 & 0.770 & 0.770 & 17.28 & 13.32 & 6.217 \\
 &  & 10 & 0.595 & 0.772 & 0.776 & 17.25 & 13.30 & 6.206 \\
\midrule
SG (loc) & gate $\tilde\Phi$ & off & 0.614 & 0.696 & 0.628 & 18.19 & 15.00 & 7.050 \\
 &  & \textbf{on} & 0.597 & 0.770 & 0.770 & 17.28 & 13.32 & 6.217 \\
\end{longtable}


==> tables/generated/ablations_vit_b16_longtable.tex <==
\begin{longtable}{@{}l l c c c c c c c@{}}
\toprule
Center & Factor & Value & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ \\
\midrule
\endfirsthead
\toprule
Center & Factor & Value & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ \\
\midrule
\endhead
\bottomrule
\endlastfoot
RG (faith) & $\tau$ & 0.3 & 0.705 & 0.802 & 0.731 & 8.34 & 7.60 & 5.195 \\
 &  & 0.4 & 0.688 & 0.827 & 0.773 & 8.26 & 7.41 & 5.095 \\
 &  & 0.5 & 0.665 & 0.821 & 0.793 & 8.22 & 7.20 & 4.956 \\
 &  & 0.6 & 0.613 & 0.814 & 0.774 & 8.13 & 6.88 & 4.820 \\
 &  & \textbf{0.7} & 0.549 & 0.770 & 0.741 & 8.11 & 6.78 & 4.808 \\
 &  & 0.8 & 0.507 & 0.742 & 0.712 & 8.14 & 6.85 & 4.881 \\
 &  & 0.9 & 0.482 & 0.697 & 0.683 & 8.21 & 7.02 & 4.983 \\
 &  & 1 & 0.467 & 0.648 & 0.648 & 8.29 & 7.25 & 5.115 \\
\midrule
RG (faith) & $\lambda_{\mathrm{sm}}$ & {-}50 & 0.467 & 0.556 & 0.541 & 8.51 & 8.13 & 5.928 \\
 &  & {-}10 & 0.556 & 0.777 & 0.763 & 8.16 & 6.97 & 4.876 \\
 &  & \textbf{{-}5} & 0.549 & 0.770 & 0.741 & 8.11 & 6.78 & 4.808 \\
 &  & {-}2 & 0.547 & 0.743 & 0.720 & 8.11 & 6.81 & 4.793 \\
 &  & {-}1 & 0.546 & 0.733 & 0.713 & 8.11 & 6.83 & 4.794 \\
 &  & 0 & 0.546 & 0.727 & 0.706 & 8.13 & 6.87 & 4.804 \\
\midrule
RG (faith) & $\sigma^2$ & 1 & 0.558 & 0.738 & 0.703 & 8.16 & 6.90 & 4.790 \\
 &  & 2 & 0.555 & 0.743 & 0.719 & 8.13 & 6.81 & 4.783 \\
 &  & \textbf{5} & 0.549 & 0.770 & 0.741 & 8.11 & 6.78 & 4.808 \\
 &  & 10 & 0.545 & 0.765 & 0.749 & 8.12 & 6.82 & 4.833 \\
\midrule
RG (faith) & $\varepsilon$ & \textbf{0.1} & 0.549 & 0.770 & 0.741 & 8.11 & 6.78 & 4.808 \\
 &  & 0.25 & 0.595 & 0.804 & 0.778 & 8.16 & 6.95 & 4.846 \\
 &  & 0.5 & 0.621 & 0.809 & 0.792 & 8.24 & 7.21 & 4.944 \\
 &  & 1 & 0.630 & 0.812 & 0.794 & 8.29 & 7.43 & 5.051 \\
\midrule
RG (faith) & +Eq ($N{=}50$) & -- & 0.557 & 0.800 & 0.791 & 8.38 & 7.69 & 4.816 \\
\midrule
RG (loc) & $\tau$ & 0.3 & 0.723 & 0.816 & 0.746 & 8.33 & 7.64 & 5.201 \\
 &  & \textbf{0.4} & 0.711 & 0.825 & 0.788 & 8.27 & 7.48 & 5.109 \\
 &  & 0.5 & 0.691 & 0.830 & 0.812 & 8.23 & 7.31 & 4.969 \\
 &  & 0.6 & 0.632 & 0.827 & 0.801 & 8.16 & 7.00 & 4.847 \\
 &  & 0.7 & 0.556 & 0.777 & 0.763 & 8.16 & 6.97 & 4.876 \\
 &  & 0.8 & 0.506 & 0.743 & 0.715 & 8.22 & 7.13 & 5.013 \\
 &  & 0.9 & 0.477 & 0.683 & 0.673 & 8.29 & 7.28 & 5.143 \\
 &  & 1 & 0.461 & 0.628 & 0.629 & 8.36 & 7.42 & 5.247 \\
\midrule
RG (loc) & $\lambda_{\mathrm{sm}}$ & {-}50 & 0.520 & 0.543 & 0.528 & 8.52 & 7.99 & 5.745 \\
 &  & \textbf{{-}10} & 0.711 & 0.825 & 0.788 & 8.27 & 7.48 & 5.109 \\
 &  & {-}5 & 0.688 & 0.827 & 0.773 & 8.26 & 7.41 & 5.095 \\
 &  & {-}2 & 0.676 & 0.827 & 0.764 & 8.26 & 7.39 & 5.086 \\
 &  & {-}1 & 0.673 & 0.818 & 0.761 & 8.26 & 7.38 & 5.080 \\
 &  & 0 & 0.671 & 0.818 & 0.758 & 8.26 & 7.38 & 5.076 \\
\midrule
RG (loc) & $\sigma^2$ & 1 & 0.707 & 0.823 & 0.769 & 8.23 & 7.35 & 4.986 \\
 &  & 2 & 0.712 & 0.823 & 0.780 & 8.24 & 7.39 & 5.032 \\
 &  & \textbf{5} & 0.711 & 0.825 & 0.788 & 8.27 & 7.48 & 5.109 \\
 &  & 10 & 0.705 & 0.837 & 0.787 & 8.31 & 7.58 & 5.168 \\
\midrule
RG (loc) & $\varepsilon$ & \textbf{0.1} & 0.711 & 0.825 & 0.788 & 8.27 & 7.48 & 5.109 \\
 &  & 0.25 & 0.709 & 0.842 & 0.780 & 8.29 & 7.55 & 5.155 \\
 &  & 0.5 & 0.708 & 0.828 & 0.776 & 8.30 & 7.57 & 5.171 \\
 &  & 1 & 0.708 & 0.823 & 0.773 & 8.31 & 7.59 & 5.181 \\
\midrule
RG (loc) & +Eq ($N{=}50$) & -- & 0.711 & 0.846 & 0.842 & 8.38 & 7.82 & 5.077 \\
\midrule
RG+Eq (faith) & $\tau$ & 0.3 & 0.721 & 0.805 & 0.786 & 8.37 & 7.75 & 5.129 \\
 &  & 0.4 & 0.712 & 0.832 & 0.822 & 8.39 & 7.81 & 5.049 \\
 &  & 0.5 & 0.698 & 0.855 & 0.836 & 8.39 & 7.80 & 5.010 \\
 &  & 0.6 & 0.681 & 0.846 & 0.833 & 8.39 & 7.77 & 4.943 \\
 &  & \textbf{0.7} & 0.654 & 0.812 & 0.820 & 8.39 & 7.71 & 4.856 \\
 &  & 0.8 & 0.610 & 0.805 & 0.803 & 8.38 & 7.70 & 4.814 \\
 &  & 0.9 & 0.567 & 0.796 & 0.787 & 8.41 & 7.71 & 4.825 \\
 &  & 1 & 0.534 & 0.777 & 0.772 & 8.42 & 7.74 & 4.876 \\
\midrule
RG+Eq (faith) & $\lambda_{\mathrm{sm}}$ & \textbf{{-}10} & 0.654 & 0.812 & 0.820 & 8.39 & 7.71 & 4.856 \\
 &  & 0 & 0.613 & 0.814 & 0.815 & 8.37 & 7.73 & 4.914 \\
\midrule
RG+Eq (loc) & $\tau$ & 0.3 & 0.721 & 0.805 & 0.786 & 8.37 & 7.75 & 5.129 \\
 &  & 0.4 & 0.712 & 0.832 & 0.822 & 8.39 & 7.81 & 5.049 \\
 &  & \textbf{0.5} & 0.698 & 0.855 & 0.836 & 8.39 & 7.80 & 5.010 \\
 &  & 0.6 & 0.681 & 0.846 & 0.833 & 8.39 & 7.77 & 4.943 \\
 &  & 0.7 & 0.654 & 0.812 & 0.820 & 8.39 & 7.71 & 4.856 \\
 &  & 0.8 & 0.610 & 0.805 & 0.803 & 8.38 & 7.70 & 4.814 \\
 &  & 0.9 & 0.567 & 0.796 & 0.787 & 8.41 & 7.71 & 4.825 \\
 &  & 1 & 0.534 & 0.777 & 0.772 & 8.42 & 7.74 & 4.876 \\
\midrule
RG+Eq (loc) & $\lambda_{\mathrm{sm}}$ & \textbf{{-}10} & 0.698 & 0.855 & 0.836 & 8.39 & 7.80 & 5.010 \\
 &  & 0 & 0.652 & 0.848 & 0.828 & 8.40 & 7.85 & 5.073 \\
\end{longtable}


==> tables/generated/test_resnet50_ci_longtable.tex <==
\begin{longtable}{@{}l@{\hspace{2.5pt}}p{2.7cm}@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{}}
\toprule
Method & Config & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ & MaxS$\downarrow$ & AvgS$\downarrow$ \\
\midrule
\endfirsthead
\toprule
Method & Config & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ & MaxS$\downarrow$ & AvgS$\downarrow$ \\
\midrule
\endhead
\midrule
\multicolumn{10}{r}{\emph{continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
Gradient & -- & \begin{tabular}[t]{@{}c@{}}0.481\\[-1pt]{\tiny[0.459,0.504]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.556\\[-1pt]{\tiny[0.515,0.596]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.568\\[-1pt]{\tiny[0.540,0.595]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.33\\[-1pt]{\tiny[6.22,6.44]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.91\\[-1pt]{\tiny[5.78,6.04]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.027\\[-1pt]{\tiny[4.900,5.151]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.448\\[-1pt]{\tiny[1.365,1.535]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.072\\[-1pt]{\tiny[1.019,1.130]}\end{tabular} \\
SmGrad (loc) & $N{=}50,\allowbreak \sigma/\mathrm{range}{=}0.15$ & \begin{tabular}[t]{@{}c@{}}0.549\\[-1pt]{\tiny[0.530,0.569]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.789\\[-1pt]{\tiny[0.756,0.821]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.738\\[-1pt]{\tiny[0.719,0.755]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.05\\[-1pt]{\tiny[5.93,6.17]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.17\\[-1pt]{\tiny[5.02,5.31]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.429\\[-1pt]{\tiny[4.303,4.554]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.735\\[-1pt]{\tiny[0.718,0.753]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.600\\[-1pt]{\tiny[0.593,0.609]}\end{tabular} \\
SmGrad (faith) & $N{=}50,\allowbreak \sigma/\mathrm{range}{=}0.1$ & \begin{tabular}[t]{@{}c@{}}0.544\\[-1pt]{\tiny[0.525,0.564]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.773\\[-1pt]{\tiny[0.740,0.807]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.735\\[-1pt]{\tiny[0.715,0.753]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.06\\[-1pt]{\tiny[5.94,6.19]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.19\\[-1pt]{\tiny[5.04,5.34]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.489\\[-1pt]{\tiny[4.361,4.612]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.726\\[-1pt]{\tiny[0.706,0.748]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.586\\[-1pt]{\tiny[0.577,0.597]}\end{tabular} \\
IntGrad (loc) & $N_{\mathrm{steps}}{=}100$,\allowbreak  black baseline & \begin{tabular}[t]{@{}c@{}}0.510\\[-1pt]{\tiny[0.488,0.532]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.635\\[-1pt]{\tiny[0.596,0.676]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.600\\[-1pt]{\tiny[0.574,0.626]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.27\\[-1pt]{\tiny[6.16,6.38]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.83\\[-1pt]{\tiny[5.69,5.96]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.949\\[-1pt]{\tiny[4.820,5.072]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.203\\[-1pt]{\tiny[1.152,1.257]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.947\\[-1pt]{\tiny[0.917,0.979]}\end{tabular} \\
IntGrad (faith) & $N_{\mathrm{steps}}{=}50$,\allowbreak  black baseline & \begin{tabular}[t]{@{}c@{}}0.507\\[-1pt]{\tiny[0.484,0.529]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.604\\[-1pt]{\tiny[0.563,0.642]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.595\\[-1pt]{\tiny[0.568,0.622]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.28\\[-1pt]{\tiny[6.16,6.39]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.82\\[-1pt]{\tiny[5.68,5.95]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.952\\[-1pt]{\tiny[4.822,5.075]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.207\\[-1pt]{\tiny[1.157,1.261]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.951\\[-1pt]{\tiny[0.922,0.983]}\end{tabular} \\
DeepLift & Rescale & \begin{tabular}[t]{@{}c@{}}0.543\\[-1pt]{\tiny[0.523,0.564]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.727\\[-1pt]{\tiny[0.690,0.765]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.653\\[-1pt]{\tiny[0.629,0.677]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.97\\[-1pt]{\tiny[5.85,6.10]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.29\\[-1pt]{\tiny[5.15,5.43]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.515\\[-1pt]{\tiny[4.390,4.637]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.273\\[-1pt]{\tiny[1.203,1.351]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.000\\[-1pt]{\tiny[0.955,1.052]}\end{tabular} \\
LRP-$\varepsilon$ (loc) & $\varepsilon{=}0.5$ & \begin{tabular}[t]{@{}c@{}}0.603\\[-1pt]{\tiny[0.584,0.622]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.775\\[-1pt]{\tiny[0.740,0.809]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.714\\[-1pt]{\tiny[0.694,0.734]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.94\\[-1pt]{\tiny[5.81,6.06]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.14\\[-1pt]{\tiny[4.99,5.28]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.318\\[-1pt]{\tiny[4.200,4.433]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.246\\[-1pt]{\tiny[1.203,1.292]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.982\\[-1pt]{\tiny[0.960,1.006]}\end{tabular} \\
LRP-$\varepsilon$ (faith) & $\varepsilon{=}2$ & \begin{tabular}[t]{@{}c@{}}0.637\\[-1pt]{\tiny[0.618,0.656]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.699\\[-1pt]{\tiny[0.662,0.736]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.683\\[-1pt]{\tiny[0.663,0.702]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.94\\[-1pt]{\tiny[5.81,6.06]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.91\\[-1pt]{\tiny[4.76,5.05]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.280\\[-1pt]{\tiny[4.164,4.394]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.262\\[-1pt]{\tiny[1.224,1.301]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.967\\[-1pt]{\tiny[0.948,0.986]}\end{tabular} \\
LRP-$\gamma$ (loc) & $\varepsilon{=}0.5,\allowbreak \gamma{=}2$,\allowbreak  $z^{\mathcal{B}}$/$\gamma$/$\varepsilon$ composite & \begin{tabular}[t]{@{}c@{}}0.711\\[-1pt]{\tiny[0.695,0.726]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.842\\[-1pt]{\tiny[0.812,0.873]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.822\\[-1pt]{\tiny[0.807,0.836]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.69\\[-1pt]{\tiny[5.55,5.83]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.53\\[-1pt]{\tiny[4.38,4.68]}\end{tabular} & \cellapprox{\begin{tabular}[t]{@{}c@{}}3.935\textsuperscript{$\approx$}\\[-1pt]{\tiny[3.814,4.053]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}0.633\\[-1pt]{\tiny[0.601,0.666]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.486\\[-1pt]{\tiny[0.464,0.507]}\end{tabular} \\
LRP-$\gamma$ (faith) & $\varepsilon{=}0.5,\allowbreak \gamma{=}0.5$,\allowbreak  $z^{\mathcal{B}}$/$\gamma$/$\varepsilon$ composite & \begin{tabular}[t]{@{}c@{}}0.700\\[-1pt]{\tiny[0.684,0.716]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.834\\[-1pt]{\tiny[0.802,0.864]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.796\\[-1pt]{\tiny[0.781,0.812]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{5.65}\\[-1pt]{\tiny[5.51,5.79]}\end{tabular}} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{4.43}\\[-1pt]{\tiny[4.28,4.59]}\end{tabular}} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{3.931}\\[-1pt]{\tiny[3.809,4.050]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}0.745\\[-1pt]{\tiny[0.714,0.777]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.584\\[-1pt]{\tiny[0.562,0.605]}\end{tabular} \\
GCAM & \texttt{layer4} & \begin{tabular}[t]{@{}c@{}}0.664\\[-1pt]{\tiny[0.645,0.683]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.873\\[-1pt]{\tiny[0.844,0.899]}\end{tabular} & \cellapprox{\begin{tabular}[t]{@{}c@{}}0.850\textsuperscript{$\approx$}\\[-1pt]{\tiny[0.830,0.870]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}6.42\\[-1pt]{\tiny[6.32,6.52]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.15\\[-1pt]{\tiny[6.03,6.26]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.344\\[-1pt]{\tiny[4.216,4.469]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.292\\[-1pt]{\tiny[0.274,0.312]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.207\\[-1pt]{\tiny[0.195,0.220]}\end{tabular} \\
GCAM++ & \texttt{layer4} & \begin{tabular}[t]{@{}c@{}}0.627\\[-1pt]{\tiny[0.607,0.646]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.834\\[-1pt]{\tiny[0.804,0.864]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.836\\[-1pt]{\tiny[0.815,0.857]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.43\\[-1pt]{\tiny[6.34,6.52]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.18\\[-1pt]{\tiny[6.07,6.29]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.483\\[-1pt]{\tiny[4.356,4.609]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.294\\[-1pt]{\tiny[0.278,0.310]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.207\\[-1pt]{\tiny[0.197,0.219]}\end{tabular} \\
LCAM & \texttt{layer4} & \begin{tabular}[t]{@{}c@{}}0.649\\[-1pt]{\tiny[0.630,0.668]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.869\\[-1pt]{\tiny[0.841,0.897]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.851}\\[-1pt]{\tiny[0.831,0.871]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}6.44\\[-1pt]{\tiny[6.34,6.53]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.18\\[-1pt]{\tiny[6.07,6.29]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.437\\[-1pt]{\tiny[4.311,4.559]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.274}\\[-1pt]{\tiny[0.260,0.288]}\end{tabular}} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.194}\\[-1pt]{\tiny[0.184,0.204]}\end{tabular}} \\
LIME & $N{=}1000$,\allowbreak  80 superpixels,\allowbreak  ridge & \begin{tabular}[t]{@{}c@{}}0.553\\[-1pt]{\tiny[0.533,0.572]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.926\\[-1pt]{\tiny[0.903,0.947]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.716\\[-1pt]{\tiny[0.687,0.744]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.37\\[-1pt]{\tiny[6.26,6.46]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.99\\[-1pt]{\tiny[5.88,6.11]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.759\\[-1pt]{\tiny[4.630,4.881]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.916\\[-1pt]{\tiny[0.891,0.941]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.672\\[-1pt]{\tiny[0.655,0.690]}\end{tabular} \\
KernelSHAP & $N{=}2M{+}2048$,\allowbreak  80 superpixels & \begin{tabular}[t]{@{}c@{}}0.558\\[-1pt]{\tiny[0.540,0.575]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.965}\\[-1pt]{\tiny[0.949,0.979]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}0.818\\[-1pt]{\tiny[0.793,0.841]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.26\\[-1pt]{\tiny[6.16,6.36]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.81\\[-1pt]{\tiny[5.69,5.92]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.727\\[-1pt]{\tiny[4.601,4.849]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.924\\[-1pt]{\tiny[0.896,0.954]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.688\\[-1pt]{\tiny[0.670,0.708]}\end{tabular} \\
RG anchor & $\tau{=}1$ & \begin{tabular}[t]{@{}c@{}}0.693\\[-1pt]{\tiny[0.676,0.710]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.752\\[-1pt]{\tiny[0.717,0.788]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.756\\[-1pt]{\tiny[0.738,0.774]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.84\\[-1pt]{\tiny[5.70,5.97]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.71\\[-1pt]{\tiny[4.56,4.86]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.017\\[-1pt]{\tiny[3.898,4.133]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.708\\[-1pt]{\tiny[0.651,0.775]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.508\\[-1pt]{\tiny[0.481,0.541]}\end{tabular} \\
RG (loc) & $\tau{=}0.9,\allowbreak \varepsilon{=}1$ & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.719}\\[-1pt]{\tiny[0.701,0.737]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}0.763\\[-1pt]{\tiny[0.727,0.796]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.760\\[-1pt]{\tiny[0.741,0.778]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.85\\[-1pt]{\tiny[5.72,5.98]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.70\\[-1pt]{\tiny[4.55,4.85]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.047\\[-1pt]{\tiny[3.929,4.163]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.798\\[-1pt]{\tiny[0.749,0.855]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.560\\[-1pt]{\tiny[0.535,0.586]}\end{tabular} \\
RG (faith) & $\tau{=}1,\allowbreak \lambda{=}{-}1,\allowbreak \sigma^2{=}1,\allowbreak \varepsilon{=}0.25$ & \begin{tabular}[t]{@{}c@{}}0.674\\[-1pt]{\tiny[0.656,0.691]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.743\\[-1pt]{\tiny[0.708,0.779]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.738\\[-1pt]{\tiny[0.719,0.756]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.88\\[-1pt]{\tiny[5.74,6.01]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.74\\[-1pt]{\tiny[4.59,4.89]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.030\\[-1pt]{\tiny[3.911,4.144]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.685\\[-1pt]{\tiny[0.629,0.755]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.489\\[-1pt]{\tiny[0.460,0.525]}\end{tabular} \\
\end{longtable}


==> tables/generated/test_vgg16_ci_longtable.tex <==
\begin{longtable}{@{}l@{\hspace{2.5pt}}p{2.7cm}@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{}}
\toprule
Method & Config & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ & MaxS$\downarrow$ & AvgS$\downarrow$ \\
\midrule
\endfirsthead
\toprule
Method & Config & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ & MaxS$\downarrow$ & AvgS$\downarrow$ \\
\midrule
\endhead
\midrule
\multicolumn{10}{r}{\emph{continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
Gradient & -- & \begin{tabular}[t]{@{}c@{}}0.522\\[-1pt]{\tiny[0.501,0.542]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.738\\[-1pt]{\tiny[0.701,0.773]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.688\\[-1pt]{\tiny[0.665,0.711]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}14.47\\[-1pt]{\tiny[13.95,14.99]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}10.96\\[-1pt]{\tiny[10.55,11.37]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.470\\[-1pt]{\tiny[6.212,6.731]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.212\\[-1pt]{\tiny[1.162,1.269]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.947\\[-1pt]{\tiny[0.917,0.980]}\end{tabular} \\
SmGrad (loc/faith) & $N{=}50,\allowbreak \sigma/\mathrm{range}{=}0.1$ & \begin{tabular}[t]{@{}c@{}}0.533\\[-1pt]{\tiny[0.515,0.552]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.782\\[-1pt]{\tiny[0.747,0.816]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.723\\[-1pt]{\tiny[0.705,0.741]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}14.12\\[-1pt]{\tiny[13.60,14.65]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}9.24\\[-1pt]{\tiny[8.85,9.63]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.768\\[-1pt]{\tiny[5.526,6.007]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.641\\[-1pt]{\tiny[0.625,0.659]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.523\\[-1pt]{\tiny[0.515,0.531]}\end{tabular} \\
IntGrad (loc/faith) & $N_{\mathrm{steps}}{=}20$,\allowbreak  black baseline & \begin{tabular}[t]{@{}c@{}}0.550\\[-1pt]{\tiny[0.530,0.571]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.770\\[-1pt]{\tiny[0.735,0.804]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.706\\[-1pt]{\tiny[0.683,0.730]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}15.39\\[-1pt]{\tiny[14.86,15.95]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}11.89\\[-1pt]{\tiny[11.46,12.32]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.438\\[-1pt]{\tiny[6.174,6.694]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.132\\[-1pt]{\tiny[1.089,1.179]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.917\\[-1pt]{\tiny[0.890,0.945]}\end{tabular} \\
DeepLift & Rescale & \begin{tabular}[t]{@{}c@{}}0.542\\[-1pt]{\tiny[0.523,0.562]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.701\\[-1pt]{\tiny[0.664,0.738]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.654\\[-1pt]{\tiny[0.631,0.677]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}13.05\\[-1pt]{\tiny[12.59,13.52]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}9.32\\[-1pt]{\tiny[8.96,9.69]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.049\\[-1pt]{\tiny[5.806,6.291]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.193\\[-1pt]{\tiny[1.145,1.249]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.948\\[-1pt]{\tiny[0.919,0.985]}\end{tabular} \\
LRP-$\varepsilon$ (loc) & $\varepsilon{=}0.5$ & \begin{tabular}[t]{@{}c@{}}0.613\\[-1pt]{\tiny[0.595,0.632]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.832\\[-1pt]{\tiny[0.800,0.862]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.745\\[-1pt]{\tiny[0.725,0.764]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}12.63\\[-1pt]{\tiny[12.18,13.10]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.61\\[-1pt]{\tiny[8.26,8.96]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.685\\[-1pt]{\tiny[5.458,5.908]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.173\\[-1pt]{\tiny[1.127,1.223]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.918\\[-1pt]{\tiny[0.893,0.947]}\end{tabular} \\
LRP-$\varepsilon$ (faith) & $\varepsilon{=}1$ & \begin{tabular}[t]{@{}c@{}}0.639\\[-1pt]{\tiny[0.621,0.657]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.809\\[-1pt]{\tiny[0.777,0.841]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.744\\[-1pt]{\tiny[0.725,0.762]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{12.43}\\[-1pt]{\tiny[11.98,12.89]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}8.17\\[-1pt]{\tiny[7.83,8.50]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.489\\[-1pt]{\tiny[5.270,5.704]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.100\\[-1pt]{\tiny[1.059,1.143]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.840\\[-1pt]{\tiny[0.820,0.861]}\end{tabular} \\
LRP-$\gamma$ (loc) & $\varepsilon{=}0.5,\allowbreak \gamma{=}0.25$,\allowbreak  $z^{\mathcal{B}}$/$\gamma$/$\varepsilon$ composite & \begin{tabular}[t]{@{}c@{}}0.601\\[-1pt]{\tiny[0.584,0.617]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.692\\[-1pt]{\tiny[0.655,0.729]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.704\\[-1pt]{\tiny[0.687,0.721]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}14.83\\[-1pt]{\tiny[14.28,15.39]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}10.07\\[-1pt]{\tiny[9.68,10.46]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{5.010}\\[-1pt]{\tiny[4.799,5.219]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}0.515\\[-1pt]{\tiny[0.489,0.542]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.368\\[-1pt]{\tiny[0.353,0.384]}\end{tabular} \\
LRP-$\gamma$ (faith) & $\varepsilon{=}0.25,\allowbreak \gamma{=}0.1$ & \begin{tabular}[t]{@{}c@{}}0.615\\[-1pt]{\tiny[0.598,0.633]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.793\\[-1pt]{\tiny[0.759,0.827]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.698\\[-1pt]{\tiny[0.681,0.716]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}12.66\\[-1pt]{\tiny[12.18,13.13]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{7.89}\\[-1pt]{\tiny[7.56,8.23]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}5.078\\[-1pt]{\tiny[4.867,5.285]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.702\\[-1pt]{\tiny[0.675,0.733]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.561\\[-1pt]{\tiny[0.543,0.580]}\end{tabular} \\
GCAM & \texttt{features.29} & \begin{tabular}[t]{@{}c@{}}0.557\\[-1pt]{\tiny[0.538,0.576]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.830\\[-1pt]{\tiny[0.798,0.860]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.821}\\[-1pt]{\tiny[0.798,0.844]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}16.36\\[-1pt]{\tiny[15.79,16.93]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}12.47\\[-1pt]{\tiny[12.01,12.93]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.640\\[-1pt]{\tiny[5.407,5.870]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.430\\[-1pt]{\tiny[0.412,0.449]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.334\\[-1pt]{\tiny[0.320,0.349]}\end{tabular} \\
GCAM++ & \texttt{features.29} & \begin{tabular}[t]{@{}c@{}}0.551\\[-1pt]{\tiny[0.533,0.569]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.823\\[-1pt]{\tiny[0.791,0.855]}\end{tabular} & \cellapprox{\begin{tabular}[t]{@{}c@{}}0.814\textsuperscript{$\approx$}\\[-1pt]{\tiny[0.792,0.835]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}16.68\\[-1pt]{\tiny[16.09,17.27]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}12.87\\[-1pt]{\tiny[12.40,13.35]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.700\\[-1pt]{\tiny[5.462,5.938]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.314\\[-1pt]{\tiny[0.301,0.327]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.243\\[-1pt]{\tiny[0.233,0.253]}\end{tabular} \\
LCAM & \texttt{features.29} & \begin{tabular}[t]{@{}c@{}}0.544\\[-1pt]{\tiny[0.526,0.562]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.720\\[-1pt]{\tiny[0.683,0.756]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.747\\[-1pt]{\tiny[0.725,0.768]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}15.98\\[-1pt]{\tiny[15.42,16.54]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}11.48\\[-1pt]{\tiny[11.05,11.91]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.341\\[-1pt]{\tiny[5.113,5.565]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.434\\[-1pt]{\tiny[0.416,0.452]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.330\\[-1pt]{\tiny[0.319,0.341]}\end{tabular} \\
LIME & $N{=}1000$,\allowbreak  80 superpixels,\allowbreak  ridge & \begin{tabular}[t]{@{}c@{}}0.603\\[-1pt]{\tiny[0.585,0.622]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.972}\\[-1pt]{\tiny[0.958,0.984]}\end{tabular}} & \cellapprox{\begin{tabular}[t]{@{}c@{}}0.814\textsuperscript{$\approx$}\\[-1pt]{\tiny[0.790,0.837]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}16.66\\[-1pt]{\tiny[16.09,17.25]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}12.62\\[-1pt]{\tiny[12.17,13.06]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.785\\[-1pt]{\tiny[5.551,6.015]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.848\\[-1pt]{\tiny[0.816,0.882]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.621\\[-1pt]{\tiny[0.599,0.644]}\end{tabular} \\
KernelSHAP & $N{=}2M{+}2048$,\allowbreak  80 superpixels & \begin{tabular}[t]{@{}c@{}}0.559\\[-1pt]{\tiny[0.541,0.577]}\end{tabular} & \cellapprox{\begin{tabular}[t]{@{}c@{}}0.954\textsuperscript{$\approx$}\\[-1pt]{\tiny[0.936,0.970]}\end{tabular}} & \cellapprox{\begin{tabular}[t]{@{}c@{}}0.820\textsuperscript{$\approx$}\\[-1pt]{\tiny[0.795,0.844]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}16.68\\[-1pt]{\tiny[16.10,17.27]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}12.82\\[-1pt]{\tiny[12.37,13.26]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.140\\[-1pt]{\tiny[5.912,6.366]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.994\\[-1pt]{\tiny[0.955,1.035]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.736\\[-1pt]{\tiny[0.712,0.761]}\end{tabular} \\
SG (loc) & $\lambda{=}{-}1,\allowbreak \sigma^2{=}5$,\allowbreak  gate on & \begin{tabular}[t]{@{}c@{}}0.597\\[-1pt]{\tiny[0.577,0.616]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.770\\[-1pt]{\tiny[0.735,0.804]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.770\\[-1pt]{\tiny[0.747,0.793]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}17.28\\[-1pt]{\tiny[16.69,17.87]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}13.32\\[-1pt]{\tiny[12.85,13.79]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.217\\[-1pt]{\tiny[5.969,6.459]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.278}\\[-1pt]{\tiny[0.267,0.290]}\end{tabular}} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.196}\\[-1pt]{\tiny[0.188,0.204]}\end{tabular}} \\
SG (faith) & $\lambda{=}{-}0.3,\allowbreak \sigma^2{=}1$,\allowbreak  gate off & \begin{tabular}[t]{@{}c@{}}0.598\\[-1pt]{\tiny[0.577,0.618]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.821\\[-1pt]{\tiny[0.789,0.851]}\end{tabular} & \cellapprox{\begin{tabular}[t]{@{}c@{}}0.788\textsuperscript{$\approx$}\\[-1pt]{\tiny[0.764,0.812]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}17.08\\[-1pt]{\tiny[16.50,17.67]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}12.98\\[-1pt]{\tiny[12.53,13.44]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.278\\[-1pt]{\tiny[6.025,6.524]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.543\\[-1pt]{\tiny[0.516,0.571]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.423\\[-1pt]{\tiny[0.401,0.446]}\end{tabular} \\
RG anchor & $\tau{=}1$ & \begin{tabular}[t]{@{}c@{}}0.619\\[-1pt]{\tiny[0.601,0.637]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.759\\[-1pt]{\tiny[0.724,0.795]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.691\\[-1pt]{\tiny[0.673,0.709]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}14.27\\[-1pt]{\tiny[13.74,14.80]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}9.49\\[-1pt]{\tiny[9.10,9.89]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.179\\[-1pt]{\tiny[4.968,5.388]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.551\\[-1pt]{\tiny[0.526,0.578]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.398\\[-1pt]{\tiny[0.385,0.412]}\end{tabular} \\
RG (loc) & $\tau{=}0.3,\allowbreak \varepsilon{=}0.1$ & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.685}\\[-1pt]{\tiny[0.665,0.705]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}0.736\\[-1pt]{\tiny[0.699,0.772]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.673\\[-1pt]{\tiny[0.654,0.692]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}14.48\\[-1pt]{\tiny[13.95,15.02]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}9.64\\[-1pt]{\tiny[9.25,10.03]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.632\\[-1pt]{\tiny[5.411,5.845]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.349\\[-1pt]{\tiny[1.273,1.430]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.879\\[-1pt]{\tiny[0.842,0.918]}\end{tabular} \\
RG (faith) & $\tau{=}0.8,\allowbreak \varepsilon{=}0.1$ & \begin{tabular}[t]{@{}c@{}}0.640\\[-1pt]{\tiny[0.623,0.658]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.712\\[-1pt]{\tiny[0.673,0.749]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.688\\[-1pt]{\tiny[0.670,0.706]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}14.05\\[-1pt]{\tiny[13.53,14.58]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}9.07\\[-1pt]{\tiny[8.70,9.46]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.117\\[-1pt]{\tiny[4.906,5.325]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.655\\[-1pt]{\tiny[0.621,0.690]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.466\\[-1pt]{\tiny[0.448,0.485]}\end{tabular} \\
\end{longtable}


==> tables/generated/test_vit_b16_ci_longtable.tex <==
\begin{longtable}{@{}l@{\hspace{2.5pt}}p{2.7cm}@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{}}
\toprule
Method & Config & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ & MaxS$\downarrow$ & AvgS$\downarrow$ \\
\midrule
\endfirsthead
\toprule
Method & Config & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ & MaxS$\downarrow$ & AvgS$\downarrow$ \\
\midrule
\endhead
\midrule
\multicolumn{10}{r}{\emph{continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
Gradient & -- & \begin{tabular}[t]{@{}c@{}}0.411\\[-1pt]{\tiny[0.389,0.432]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.361\\[-1pt]{\tiny[0.322,0.402]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.386\\[-1pt]{\tiny[0.359,0.413]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.45\\[-1pt]{\tiny[8.33,8.56]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.08\\[-1pt]{\tiny[7.94,8.22]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.033\\[-1pt]{\tiny[5.905,6.154]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.290\\[-1pt]{\tiny[1.233,1.351]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.922\\[-1pt]{\tiny[0.893,0.953]}\end{tabular} \\
SmGrad (loc/faith) & $N{=}50,\allowbreak \sigma/\mathrm{range}{=}0.2$ & \begin{tabular}[t]{@{}c@{}}0.517\\[-1pt]{\tiny[0.498,0.536]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.706\\[-1pt]{\tiny[0.667,0.743]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.675\\[-1pt]{\tiny[0.654,0.694]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.10\\[-1pt]{\tiny[7.96,8.24]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.02\\[-1pt]{\tiny[6.83,7.20]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.029\\[-1pt]{\tiny[4.894,5.163]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.597\\[-1pt]{\tiny[0.569,0.630]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.468\\[-1pt]{\tiny[0.451,0.485]}\end{tabular} \\
IntGrad (loc/faith) & $N_{\mathrm{steps}}{=}100$,\allowbreak  black baseline & \begin{tabular}[t]{@{}c@{}}0.458\\[-1pt]{\tiny[0.437,0.479]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.513\\[-1pt]{\tiny[0.473,0.554]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.498\\[-1pt]{\tiny[0.472,0.524]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.37\\[-1pt]{\tiny[8.24,8.48]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.93\\[-1pt]{\tiny[7.78,8.08]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.712\\[-1pt]{\tiny[5.577,5.842]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.090\\[-1pt]{\tiny[1.041,1.140]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.825\\[-1pt]{\tiny[0.796,0.855]}\end{tabular} \\
LRP-$\varepsilon$ (loc) & $\varepsilon{=}0.25$ & \begin{tabular}[t]{@{}c@{}}0.592\\[-1pt]{\tiny[0.575,0.610]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.834\\[-1pt]{\tiny[0.804,0.864]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.746\\[-1pt]{\tiny[0.728,0.764]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.97\\[-1pt]{\tiny[7.81,8.11]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.88\\[-1pt]{\tiny[6.69,7.07]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.859\\[-1pt]{\tiny[4.733,4.983]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.486\\[-1pt]{\tiny[0.468,0.505]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.384\\[-1pt]{\tiny[0.372,0.395]}\end{tabular} \\
LRP-$\varepsilon$ (faith) & $\varepsilon{=}0.1$ & \begin{tabular}[t]{@{}c@{}}0.582\\[-1pt]{\tiny[0.564,0.599]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.834\\[-1pt]{\tiny[0.804,0.864]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.748\\[-1pt]{\tiny[0.730,0.765]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.84\\[-1pt]{\tiny[7.68,7.99]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.76\\[-1pt]{\tiny[6.57,6.96]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.890\\[-1pt]{\tiny[4.763,5.015]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.623\\[-1pt]{\tiny[0.597,0.650]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.498\\[-1pt]{\tiny[0.482,0.515]}\end{tabular} \\
LRP-$\gamma$ (loc) & $\varepsilon{=}0.1,\allowbreak \gamma{=}2$ & \begin{tabular}[t]{@{}c@{}}0.644\\[-1pt]{\tiny[0.628,0.660]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.873\\[-1pt]{\tiny[0.844,0.899]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.816\\[-1pt]{\tiny[0.800,0.832]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.93\\[-1pt]{\tiny[7.78,8.08]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.64\\[-1pt]{\tiny[6.44,6.83]}\end{tabular} & \cellapprox{\begin{tabular}[t]{@{}c@{}}4.451\textsuperscript{$\approx$}\\[-1pt]{\tiny[4.324,4.572]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}0.300\\[-1pt]{\tiny[0.287,0.314]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.218\\[-1pt]{\tiny[0.210,0.226]}\end{tabular} \\
LRP-$\gamma$ (faith) & $\varepsilon{=}0.1,\allowbreak \gamma{=}0.1$ & \begin{tabular}[t]{@{}c@{}}0.614\\[-1pt]{\tiny[0.597,0.630]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.844\\[-1pt]{\tiny[0.814,0.873]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.779\\[-1pt]{\tiny[0.763,0.795]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.73\\[-1pt]{\tiny[7.56,7.89]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.40\\[-1pt]{\tiny[6.20,6.60]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.603\\[-1pt]{\tiny[4.478,4.724]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.394\\[-1pt]{\tiny[0.378,0.410]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.309\\[-1pt]{\tiny[0.299,0.319]}\end{tabular} \\
AttnLRP (loc) & $\gamma_{\mathrm{conv}}{=}0.25,\allowbreak \gamma_{\mathrm{lin}}{=}0.05,\allowbreak \varepsilon_{\mathrm{attn}}{=}0.25$ & \begin{tabular}[t]{@{}c@{}}0.644\\[-1pt]{\tiny[0.628,0.660]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.855\\[-1pt]{\tiny[0.825,0.883]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.809\\[-1pt]{\tiny[0.794,0.825]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.77\\[-1pt]{\tiny[7.61,7.93]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.43\\[-1pt]{\tiny[6.23,6.62]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.582\\[-1pt]{\tiny[4.452,4.706]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.456\\[-1pt]{\tiny[0.430,0.484]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.342\\[-1pt]{\tiny[0.324,0.364]}\end{tabular} \\
AttnLRP (faith) & $\gamma_{\mathrm{conv}}{=}0.25,\allowbreak \gamma_{\mathrm{lin}}{=}0.05,\allowbreak \varepsilon_{\mathrm{attn}}{=}0.01$ & \begin{tabular}[t]{@{}c@{}}0.629\\[-1pt]{\tiny[0.613,0.645]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.850\\[-1pt]{\tiny[0.819,0.878]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.798\\[-1pt]{\tiny[0.783,0.814]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{7.64}\\[-1pt]{\tiny[7.47,7.81]}\end{tabular}} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{6.12}\\[-1pt]{\tiny[5.92,6.32]}\end{tabular}} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{4.441}\\[-1pt]{\tiny[4.314,4.563]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}0.416\\[-1pt]{\tiny[0.395,0.438]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.317\\[-1pt]{\tiny[0.304,0.331]}\end{tabular} \\
DAVE (loc/faith) & $N{=}50,\allowbreak \theta_{\max}{=}0,\allowbreak s_{\max}{=}0,\allowbreak t_{\max}{=}0.5$ & \begin{tabular}[t]{@{}c@{}}0.491\\[-1pt]{\tiny[0.472,0.510]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.717\\[-1pt]{\tiny[0.678,0.752]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.612\\[-1pt]{\tiny[0.591,0.633]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.12\\[-1pt]{\tiny[7.98,8.25]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.37\\[-1pt]{\tiny[7.19,7.54]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.386\\[-1pt]{\tiny[5.256,5.514]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.781\\[-1pt]{\tiny[0.755,0.810]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.643\\[-1pt]{\tiny[0.626,0.661]}\end{tabular} \\
TIBAV & -- & \begin{tabular}[t]{@{}c@{}}0.615\\[-1pt]{\tiny[0.597,0.634]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.878\\[-1pt]{\tiny[0.851,0.904]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.782\\[-1pt]{\tiny[0.759,0.805]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.13\\[-1pt]{\tiny[8.01,8.24]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.60\\[-1pt]{\tiny[7.46,7.74]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.906\\[-1pt]{\tiny[4.774,5.033]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.062\\[-1pt]{\tiny[1.001,1.126]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.512\\[-1pt]{\tiny[0.486,0.540]}\end{tabular} \\
GAE & -- & \begin{tabular}[t]{@{}c@{}}0.533\\[-1pt]{\tiny[0.514,0.551]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.743\\[-1pt]{\tiny[0.708,0.779]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.649\\[-1pt]{\tiny[0.623,0.677]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.13\\[-1pt]{\tiny[8.01,8.25]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.62\\[-1pt]{\tiny[7.47,7.76]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.098\\[-1pt]{\tiny[4.961,5.231]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.525\\[-1pt]{\tiny[0.494,0.558]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.368\\[-1pt]{\tiny[0.346,0.391]}\end{tabular} \\
AR (loc/faith) & $w_r{=}0.75$ & \begin{tabular}[t]{@{}c@{}}0.447\\[-1pt]{\tiny[0.428,0.467]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.565\\[-1pt]{\tiny[0.522,0.605]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.537\\[-1pt]{\tiny[0.510,0.564]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.44\\[-1pt]{\tiny[8.34,8.53]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.06\\[-1pt]{\tiny[7.94,8.17]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.254\\[-1pt]{\tiny[5.128,5.374]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.208\\[-1pt]{\tiny[0.195,0.222]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.122\\[-1pt]{\tiny[0.116,0.128]}\end{tabular} \\
LIME & $N{=}1000$,\allowbreak  80 superpixels,\allowbreak  ridge & \begin{tabular}[t]{@{}c@{}}0.535\\[-1pt]{\tiny[0.515,0.553]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.897\\[-1pt]{\tiny[0.871,0.922]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.686\\[-1pt]{\tiny[0.656,0.716]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.36\\[-1pt]{\tiny[8.25,8.46]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.68\\[-1pt]{\tiny[7.54,7.82]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.376\\[-1pt]{\tiny[5.242,5.505]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.937\\[-1pt]{\tiny[0.905,0.972]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.668\\[-1pt]{\tiny[0.647,0.689]}\end{tabular} \\
KernelSHAP & $N{=}2M{+}2048$,\allowbreak  80 superpixels & \begin{tabular}[t]{@{}c@{}}0.565\\[-1pt]{\tiny[0.548,0.583]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.961}\\[-1pt]{\tiny[0.945,0.977]}\end{tabular}} & \cellapprox{\begin{tabular}[t]{@{}c@{}}0.823\textsuperscript{$\approx$}\\[-1pt]{\tiny[0.799,0.848]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}8.29\\[-1pt]{\tiny[8.18,8.40]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.50\\[-1pt]{\tiny[7.35,7.65]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.140\\[-1pt]{\tiny[5.012,5.261]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.897\\[-1pt]{\tiny[0.868,0.928]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.650\\[-1pt]{\tiny[0.632,0.667]}\end{tabular} \\
RG anchor & $\tau{=}1$ & \begin{tabular}[t]{@{}c@{}}0.509\\[-1pt]{\tiny[0.490,0.528]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.724\\[-1pt]{\tiny[0.685,0.759]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.699\\[-1pt]{\tiny[0.678,0.720]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.19\\[-1pt]{\tiny[8.05,8.31]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.97\\[-1pt]{\tiny[6.78,7.15]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.854\\[-1pt]{\tiny[4.732,4.972]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.166}\\[-1pt]{\tiny[0.161,0.172]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}0.120\\[-1pt]{\tiny[0.117,0.124]}\end{tabular} \\
RG (loc) & $\tau{=}0.4,\allowbreak \lambda_{\mathrm{sm}}{=}{-}10,\allowbreak \sigma^2{=}5,\allowbreak \varepsilon{=}0.1$ & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.711}\\[-1pt]{\tiny[0.692,0.730]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}0.825\\[-1pt]{\tiny[0.793,0.855]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.788\\[-1pt]{\tiny[0.768,0.808]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.27\\[-1pt]{\tiny[8.14,8.39]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.48\\[-1pt]{\tiny[7.31,7.64]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.109\\[-1pt]{\tiny[4.987,5.226]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.729\\[-1pt]{\tiny[0.685,0.777]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.494\\[-1pt]{\tiny[0.471,0.518]}\end{tabular} \\
RG (faith) & $\tau{=}0.7,\allowbreak \lambda_{\mathrm{sm}}{=}{-}5,\allowbreak \sigma^2{=}5,\allowbreak \varepsilon{=}0.1$ & \begin{tabular}[t]{@{}c@{}}0.549\\[-1pt]{\tiny[0.531,0.567]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.770\\[-1pt]{\tiny[0.736,0.804]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.741\\[-1pt]{\tiny[0.721,0.760]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.11\\[-1pt]{\tiny[7.97,8.24]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}6.78\\[-1pt]{\tiny[6.59,6.97]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.808\\[-1pt]{\tiny[4.686,4.925]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.257\\[-1pt]{\tiny[0.245,0.268]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.174\\[-1pt]{\tiny[0.168,0.179]}\end{tabular} \\
RG+Eq anchor & $\tau{=}1,\allowbreak N{=}50$ & \begin{tabular}[t]{@{}c@{}}0.520\\[-1pt]{\tiny[0.501,0.539]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.761\\[-1pt]{\tiny[0.726,0.796]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.752\\[-1pt]{\tiny[0.729,0.775]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.41\\[-1pt]{\tiny[8.29,8.52]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.72\\[-1pt]{\tiny[7.56,7.87]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.864\\[-1pt]{\tiny[4.742,4.981]}\end{tabular} & \cellapprox{\begin{tabular}[t]{@{}c@{}}0.170\textsuperscript{$\approx$}\\[-1pt]{\tiny[0.165,0.175]}\end{tabular}} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.115}\\[-1pt]{\tiny[0.112,0.118]}\end{tabular}} \\
RG+Eq (loc) & $\tau{=}0.5,\allowbreak \lambda_{\mathrm{sm}}{=}{-}10,\allowbreak \sigma^2{=}2,\allowbreak N{=}50$ & \begin{tabular}[t]{@{}c@{}}0.698\\[-1pt]{\tiny[0.680,0.717]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.855\\[-1pt]{\tiny[0.827,0.883]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.836}\\[-1pt]{\tiny[0.815,0.857]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}8.39\\[-1pt]{\tiny[8.28,8.50]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.80\\[-1pt]{\tiny[7.65,7.94]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}5.010\\[-1pt]{\tiny[4.889,5.127]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.441\\[-1pt]{\tiny[0.421,0.463]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.301\\[-1pt]{\tiny[0.290,0.313]}\end{tabular} \\
RG+Eq (faith) & $\tau{=}0.7,\allowbreak \lambda_{\mathrm{sm}}{=}{-}10,\allowbreak \sigma^2{=}2,\allowbreak N{=}50$ & \begin{tabular}[t]{@{}c@{}}0.654\\[-1pt]{\tiny[0.636,0.672]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.812\\[-1pt]{\tiny[0.781,0.844]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.820\\[-1pt]{\tiny[0.799,0.841]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}8.39\\[-1pt]{\tiny[8.28,8.51]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}7.71\\[-1pt]{\tiny[7.56,7.86]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}4.856\\[-1pt]{\tiny[4.735,4.974]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.310\\[-1pt]{\tiny[0.297,0.325]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.199\\[-1pt]{\tiny[0.194,0.206]}\end{tabular} \\
\end{longtable}


==> tables/generated/test_voc_vit_b16_ci_longtable.tex <==
\begin{longtable}{@{}l@{\hspace{2.5pt}}p{2.7cm}@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{\hspace{2.5pt}}c@{}}
\toprule
Method & Config & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ & MaxS$\downarrow$ & AvgS$\downarrow$ \\
\midrule
\endfirsthead
\toprule
Method & Config & AL$\uparrow$ & PG$\uparrow$ & TK$\uparrow$ & PF$_5$$\downarrow$ & PF$_{20}$$\downarrow$ & Sel$\downarrow$ & MaxS$\downarrow$ & AvgS$\downarrow$ \\
\midrule
\endhead
\midrule
\multicolumn{10}{r}{\emph{continued on next page}} \\
\endfoot
\bottomrule
\endlastfoot
Gradient & -- & \begin{tabular}[t]{@{}c@{}}0.295\\[-1pt]{\tiny[0.286,0.304]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.360\\[-1pt]{\tiny[0.343,0.378]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.355\\[-1pt]{\tiny[0.344,0.367]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.45\\[-1pt]{\tiny[3.32,3.57]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.17\\[-1pt]{\tiny[3.05,3.28]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.316\\[-1pt]{\tiny[2.234,2.398]}\end{tabular} & -- & -- \\
SmGrad (loc) & $N{=}50,\allowbreak \sigma/\mathrm{range}{=}0.1$ & \begin{tabular}[t]{@{}c@{}}0.344\\[-1pt]{\tiny[0.335,0.353]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.557\\[-1pt]{\tiny[0.539,0.576]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.511\\[-1pt]{\tiny[0.500,0.521]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.25\\[-1pt]{\tiny[3.13,3.37]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.70\\[-1pt]{\tiny[2.60,2.81]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.940\\[-1pt]{\tiny[1.870,2.010]}\end{tabular} & -- & -- \\
SmGrad (faith) & $N{=}50,\allowbreak \sigma/\mathrm{range}{=}0.15$ & \begin{tabular}[t]{@{}c@{}}0.347\\[-1pt]{\tiny[0.338,0.355]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.555\\[-1pt]{\tiny[0.537,0.574]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.511\\[-1pt]{\tiny[0.500,0.522]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.24\\[-1pt]{\tiny[3.12,3.35]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.67\\[-1pt]{\tiny[2.57,2.77]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.907\\[-1pt]{\tiny[1.841,1.975]}\end{tabular} & -- & -- \\
IntGrad (loc) & $N_{\mathrm{steps}}{=}300$,\allowbreak  black baseline & \begin{tabular}[t]{@{}c@{}}0.292\\[-1pt]{\tiny[0.283,0.301]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.388\\[-1pt]{\tiny[0.369,0.406]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.358\\[-1pt]{\tiny[0.346,0.369]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.43\\[-1pt]{\tiny[3.31,3.56]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.21\\[-1pt]{\tiny[3.10,3.32]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.278\\[-1pt]{\tiny[2.197,2.356]}\end{tabular} & -- & -- \\
IntGrad (faith) & $N_{\mathrm{steps}}{=}100$,\allowbreak  black baseline & \begin{tabular}[t]{@{}c@{}}0.292\\[-1pt]{\tiny[0.283,0.301]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.389\\[-1pt]{\tiny[0.370,0.407]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.358\\[-1pt]{\tiny[0.346,0.369]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.44\\[-1pt]{\tiny[3.31,3.56]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.21\\[-1pt]{\tiny[3.10,3.32]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.279\\[-1pt]{\tiny[2.198,2.357]}\end{tabular} & -- & -- \\
LRP-$\varepsilon$ (loc/faith) & $\varepsilon{=}0.1$ & \begin{tabular}[t]{@{}c@{}}0.378\\[-1pt]{\tiny[0.368,0.387]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.604\\[-1pt]{\tiny[0.586,0.622]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.518\\[-1pt]{\tiny[0.507,0.529]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.07\\[-1pt]{\tiny[2.96,3.19]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.63\\[-1pt]{\tiny[2.54,2.73]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.923\\[-1pt]{\tiny[1.857,1.990]}\end{tabular} & -- & -- \\
LRP-$\gamma$ (loc/faith) & $\varepsilon{=}0.1,\allowbreak \gamma{=}1$ & \begin{tabular}[t]{@{}c@{}}0.403\\[-1pt]{\tiny[0.394,0.412]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.591\\[-1pt]{\tiny[0.572,0.609]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.545\\[-1pt]{\tiny[0.533,0.556]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.99\\[-1pt]{\tiny[2.88,3.10]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.37\\[-1pt]{\tiny[2.27,2.46]}\end{tabular} & \cellapprox{\begin{tabular}[t]{@{}c@{}}1.694\textsuperscript{$\approx$}\\[-1pt]{\tiny[1.634,1.756]}\end{tabular}} & -- & -- \\
AttnLRP (loc/faith) & $\gamma_{\mathrm{conv}}{=}0.25,\allowbreak \gamma_{\mathrm{lin}}{=}0.05,\allowbreak \varepsilon_{\mathrm{attn}}{=}0.05$ & \begin{tabular}[t]{@{}c@{}}0.404\\[-1pt]{\tiny[0.394,0.413]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.602\\[-1pt]{\tiny[0.583,0.620]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.542\\[-1pt]{\tiny[0.530,0.553]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{2.91}\\[-1pt]{\tiny[2.80,3.01]}\end{tabular}} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{2.31}\\[-1pt]{\tiny[2.22,2.40]}\end{tabular}} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{1.690}\\[-1pt]{\tiny[1.631,1.750]}\end{tabular}} & -- & -- \\
DAVE (loc) & $N{=}50,\allowbreak \theta_{\max}{=}0,\allowbreak s_{\max}{=}0,\allowbreak t_{\max}{=}0.25$ & \begin{tabular}[t]{@{}c@{}}0.334\\[-1pt]{\tiny[0.325,0.342]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.547\\[-1pt]{\tiny[0.529,0.565]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.456\\[-1pt]{\tiny[0.445,0.467]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.37\\[-1pt]{\tiny[3.25,3.49]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.01\\[-1pt]{\tiny[2.90,3.12]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.172\\[-1pt]{\tiny[2.097,2.247]}\end{tabular} & -- & -- \\
DAVE (faith) & $N{=}50,\allowbreak \theta_{\max}{=}0,\allowbreak s_{\max}{=}0,\allowbreak t_{\max}{=}0.5$ & \begin{tabular}[t]{@{}c@{}}0.332\\[-1pt]{\tiny[0.323,0.341]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.535\\[-1pt]{\tiny[0.517,0.553]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.454\\[-1pt]{\tiny[0.444,0.465]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.37\\[-1pt]{\tiny[3.25,3.49]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.98\\[-1pt]{\tiny[2.88,3.09]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.153\\[-1pt]{\tiny[2.080,2.226]}\end{tabular} & -- & -- \\
TIBAV & -- & \begin{tabular}[t]{@{}c@{}}0.413\\[-1pt]{\tiny[0.403,0.423]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.729\\[-1pt]{\tiny[0.713,0.746]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.575}\\[-1pt]{\tiny[0.561,0.589]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}3.04\\[-1pt]{\tiny[2.92,3.15]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.67\\[-1pt]{\tiny[2.56,2.78]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.731\\[-1pt]{\tiny[1.666,1.798]}\end{tabular} & -- & -- \\
GAE & -- & \begin{tabular}[t]{@{}c@{}}0.355\\[-1pt]{\tiny[0.346,0.364]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.712\\[-1pt]{\tiny[0.695,0.729]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.548\\[-1pt]{\tiny[0.535,0.561]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.00\\[-1pt]{\tiny[2.88,3.11]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.63\\[-1pt]{\tiny[2.52,2.74]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.754\\[-1pt]{\tiny[1.685,1.823]}\end{tabular} & -- & -- \\
AR (loc/faith) & $w_r{=}0.75$ & \begin{tabular}[t]{@{}c@{}}0.272\\[-1pt]{\tiny[0.264,0.281]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.471\\[-1pt]{\tiny[0.452,0.489]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.411\\[-1pt]{\tiny[0.398,0.424]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.57\\[-1pt]{\tiny[3.45,3.68]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.41\\[-1pt]{\tiny[3.30,3.51]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.146\\[-1pt]{\tiny[2.075,2.216]}\end{tabular} & -- & -- \\
LIME & $N{=}1000$,\allowbreak  80 superpixels,\allowbreak  ridge & \begin{tabular}[t]{@{}c@{}}0.351\\[-1pt]{\tiny[0.342,0.360]}\end{tabular} & \cellapprox{\begin{tabular}[t]{@{}c@{}}0.785\textsuperscript{$\approx$}\\[-1pt]{\tiny[0.769,0.799]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}0.523\\[-1pt]{\tiny[0.508,0.537]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.45\\[-1pt]{\tiny[3.33,3.56]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.21\\[-1pt]{\tiny[3.11,3.32]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.121\\[-1pt]{\tiny[2.051,2.191]}\end{tabular} & -- & -- \\
KernelSHAP & $N{=}2M{+}2048$,\allowbreak  80 superpixels & \begin{tabular}[t]{@{}c@{}}0.341\\[-1pt]{\tiny[0.332,0.350]}\end{tabular} & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.793}\\[-1pt]{\tiny[0.778,0.808]}\end{tabular}} & \cellapprox{\begin{tabular}[t]{@{}c@{}}0.561\textsuperscript{$\approx$}\\[-1pt]{\tiny[0.546,0.576]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}3.36\\[-1pt]{\tiny[3.25,3.48]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.03\\[-1pt]{\tiny[2.93,3.13]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.077\\[-1pt]{\tiny[2.009,2.147]}\end{tabular} & -- & -- \\
RG anchor & $\tau{=}1$ & \begin{tabular}[t]{@{}c@{}}0.323\\[-1pt]{\tiny[0.314,0.332]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.517\\[-1pt]{\tiny[0.498,0.536]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.489\\[-1pt]{\tiny[0.477,0.501]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.30\\[-1pt]{\tiny[3.18,3.41]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.67\\[-1pt]{\tiny[2.57,2.77]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.980\\[-1pt]{\tiny[1.914,2.046]}\end{tabular} & -- & -- \\
RG (loc) & $\tau{=}0.4,\allowbreak \lambda_{\mathrm{sm}}{=}{-}10,\allowbreak \sigma^2{=}5,\allowbreak \varepsilon{=}0.1$ & \cellbest{\begin{tabular}[t]{@{}c@{}}\textbf{0.459}\\[-1pt]{\tiny[0.448,0.471]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}0.562\\[-1pt]{\tiny[0.544,0.580]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.512\\[-1pt]{\tiny[0.500,0.526]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.44\\[-1pt]{\tiny[3.33,3.56]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.06\\[-1pt]{\tiny[2.96,3.17]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.152\\[-1pt]{\tiny[2.082,2.222]}\end{tabular} & -- & -- \\
RG (faith) & $\tau{=}0.7,\allowbreak \lambda_{\mathrm{sm}}{=}{-}5,\allowbreak \sigma^2{=}5,\allowbreak \varepsilon{=}0.1$ & \begin{tabular}[t]{@{}c@{}}0.351\\[-1pt]{\tiny[0.342,0.360]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.538\\[-1pt]{\tiny[0.520,0.557]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.508\\[-1pt]{\tiny[0.496,0.520]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.27\\[-1pt]{\tiny[3.15,3.38]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.63\\[-1pt]{\tiny[2.53,2.73]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.965\\[-1pt]{\tiny[1.900,2.032]}\end{tabular} & -- & -- \\
RG+Eq anchor & $\tau{=}1,\allowbreak N{=}50$ & \begin{tabular}[t]{@{}c@{}}0.329\\[-1pt]{\tiny[0.320,0.338]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.574\\[-1pt]{\tiny[0.556,0.592]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.534\\[-1pt]{\tiny[0.521,0.548]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.43\\[-1pt]{\tiny[3.31,3.55]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.06\\[-1pt]{\tiny[2.95,3.17]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}1.988\\[-1pt]{\tiny[1.922,2.055]}\end{tabular} & -- & -- \\
RG+Eq (loc) & $\tau{=}0.5,\allowbreak \lambda_{\mathrm{sm}}{=}{-}10,\allowbreak \sigma^2{=}2,\allowbreak N{=}50$ & \begin{tabular}[t]{@{}c@{}}0.456\\[-1pt]{\tiny[0.445,0.467]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.599\\[-1pt]{\tiny[0.581,0.617]}\end{tabular} & \cellapprox{\begin{tabular}[t]{@{}c@{}}0.571\textsuperscript{$\approx$}\\[-1pt]{\tiny[0.556,0.585]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}3.45\\[-1pt]{\tiny[3.33,3.57]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.14\\[-1pt]{\tiny[3.03,3.25]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.085\\[-1pt]{\tiny[2.017,2.154]}\end{tabular} & -- & -- \\
RG+Eq (faith) & $\tau{=}0.7,\allowbreak \lambda_{\mathrm{sm}}{=}{-}10,\allowbreak \sigma^2{=}2,\allowbreak N{=}50$ & \begin{tabular}[t]{@{}c@{}}0.424\\[-1pt]{\tiny[0.414,0.434]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}0.591\\[-1pt]{\tiny[0.573,0.609]}\end{tabular} & \cellapprox{\begin{tabular}[t]{@{}c@{}}0.562\textsuperscript{$\approx$}\\[-1pt]{\tiny[0.548,0.576]}\end{tabular}} & \begin{tabular}[t]{@{}c@{}}3.44\\[-1pt]{\tiny[3.32,3.55]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}3.08\\[-1pt]{\tiny[2.98,3.19]}\end{tabular} & \begin{tabular}[t]{@{}c@{}}2.004\\[-1pt]{\tiny[1.937,2.071]}\end{tabular} & -- & -- \\
\end{longtable}

